Two-Stream Aural-Visual Affect Analysis in the Wild

Human affect recognition is an essential part of natural human-computer interaction. However, current methods are still in their infancy, especially for in-the-wild data. In this work, we introduce our submission to the Affective Behavior Analysis in-the-wild (ABAW) 2020 competition. We propose a two-stream aural-visual analysis model to recognize affective behavior from videos. Audio and image streams are first processed separately and fed into a convolutional neural network. Instead of applying recurrent architectures for temporal analysis we only use temporal convolutions. Furthermore, the model is given access to additional features extracted during face-alignment. At training time, we exploit correlations between different emotion representations to improve performance. Our model achieves promising results on the challenging Aff-Wild2 database.

==> table.tex <==
\begin{table*}[tb]
%\captionsetup{font=small}
\caption{Results on Aff-Wild2 validation set}
% compared to the results from \cite{kollias2020ABAWCompetition}

\begin{center}
\def\arraystretch{1.1}
\begin{tabular}{lrrrrr}
\hline
Method & CCC Valence & CCC Arousal & CCC Mean & Expression Criterion & Action Unit Criterion \\
\hline\hline
Baselines from \cite{kollias2020ABAWCompetition}: &  &  &  &  & \\
PatchGAN & 0.14 & 0.24 & 0.19 & - & -\\
MobileNetV2 & - & - & - & 0.36 & - \\
MobileNetV2 & - & - & - & - & 0.31 \\
\hline
Other contestants & - & - & - & - & - \\
TSAV (Ours) & 0.493 & 0.613 & 0.553 & 0.546 & 0.587\\
\hline

\end{tabular}
\end{center}

\label{tab:results}
\end{table*}
